One Bad Apple Spoils the Barrel: Understanding the Security Risks Introduced by Third-Party Components in IoT Firmware

Currently, the development of IoT firmware heavily depends on third-party components (TPCs) to improve development efficiency. Nevertheless, TPCs are not secure, and the vulnerabilities in TPCs will influence the security of IoT firmware. Existing works pay less attention to the vulnerabilities caused by TPCs, and we still lack a comprehensive understanding of the security impact of TPC vulnerability against firmware. To fill in the knowledge gap, we design and implement FirmSec, which leverages syntactical features and control-flow graph features to detect the TPCs in firmware, and then recognizes the corresponding vulnerabilities. Based on FirmSec, we present the first large-scale analysis of the security risks raised by TPCs on $34,136$ firmware images. We successfully detect 584 TPCs and identify 128,757 vulnerabilities caused by 429 CVEs. Our in-depth analysis reveals the diversity of security risks in firmware and discovers some well-known vulnerabilities are still rooted in firmware. Besides, we explore the geographical distribution of vulnerable devices and confirm that the security situation of devices in different regions varies. Our analysis also indicates that vulnerabilities caused by TPCs in firmware keep growing with the boom of the IoT ecosystem. Further analysis shows 2,478 commercial firmware images have potentially violated GPL/AGPL licensing terms.

==> 0x00Abstract.tex <==
\begin{abstract}
As the core of IoT devices, firmware is undoubtedly vital. Currently, the development of IoT firmware heavily depends on third-party components (TPCs), which significantly improves the development efficiency and reduces the cost. Nevertheless, TPCs are not secure~\cite{durumeric2014matter,shellshock}, and the vulnerabilities in TPCs will turn back influence the security of IoT firmware~\cite{tpciotvul}. Currently, existing works~\cite{costin2014large, chen2016towards, feng2016scalable, david2018firmup} pay less attention to the vulnerabilities caused by TPCs, and we still lack a comprehensive understanding of the security impact of TPC vulnerability against firmware. 
% The rapid booming of IoT devices raises public's concern about their security. 
% As shown in many existing works~\cite{costin2014large, chen2016towards, feng2016scalable, david2018firmup}, IoT firmware has severe security issues.
% %Nevertheless, previous works have several limitations in evaluating the security of firmware. First, less attention has been paid to discover the N-days vulnerabilities caused by the third-party components used in firmware. Second, 
% %most of them dedicate to evaluating the security of Linux based firmware and lack the discussion of smart homes, which however is one of the primary sectors of IoT.
% %Finally, existing methods are not scalable on analyzing different kinds of firmware at a large-scale due to the fragmentation of firmware.
% In particular, IoT firmware integrates third-party components (TPCs) for different functionalities, which opens up many new attack surfaces.
% Nevertheless, previous works pay less attention to the vulnerabilities caused by TPCs and existing systems are far from being able to perform a large-scale analysis on firmware due to limited scalability. Yet, we still lack a deep understanding of the TPCs used in firmware and the vulnerabilities caused by them.

% Currently, we still lack a comprehensive understanding of the third-party components used in firmware and the vulnerabilities caused by them, as well as the practical technique needed to address this problem.


% To fill in the  knowledge gap, we present the first large-scale analysis of the usage of TPCs and the corresponding vulnerabilities in firmware based on \system. \system leverages syntactical features and control-flow graph features to detect the TPCs at version-level in firmware, and then recognizes the corresponding  vulnerabilities.
To fill in the knowledge gap, we design and implement \system, which leverages syntactical features and control-flow graph features to detect the TPCs at version-level in firmware, and then recognizes the corresponding vulnerabilities. Based on \system, we present the first large-scale analysis of the usage of TPCs and the corresponding vulnerabilities in firmware.
% design and implement \system, which dedicates to discovering the TPCs used in firmware and identifying the corresponding vulnerabilities. \system leverages syntactical features and control-flow graph features to detect the TPCs at version-level in firmware, and recognizes the vulnerabilities through versions check with our TPC database. 
% % The database includes $1,942$ unique TPCs with known CVEs. 
% Based on \system, we conduct 
% We compare  \system with one academic work developed by Costin et al.~\cite{costin2014large}, and two industry-leading systems from 360~\cite{360iot} and Alibaba~\cite{aliiot}. \system detects an average of $15.8$ third-party components and $114.2$ vulnerabilities per firmware image while the corresponding numbers of \cite{costin2014large}, \textit{360}, and \textit{Alibaba} are $7.7$ and $82.9$, $4.8$ and $62.3$, $3$ and $55.5$, respectively. In addition, \system spends an average of $4.2s$ on each firmware image while \cite{costin2014large}, \textit{360}, and \textit{Alibaba} spend $303s$, $60s$, and $174.7s$, respectively.
% Based on \system, 
More specifically, we perform an analysis on $34,136$ firmware images, 
including $11,086$ publicly accessible firmware images, and $23,050$ private firmware images from 
% hundreds of vendors that intelligentized by
TSmart~\Footnotes\footnote{The anonymized name TSmart represents a world-leading company that mainly focuses on smart homes. }. We successfully detect $584$ TPCs and identify $128,757$  vulnerabilities caused by $429$ CVEs. Our in-depth analysis reveals the diversity of security issues for different kinds of firmware from various vendors, and discovers some well-known vulnerabilities are still deeply rooted in many firmware images.
% confirm that the firmware of router is most vulnerable and the firmware from Xiaomi, one leading IoT company, is most dangerous. 
We also find that the TPCs used in firmware have fallen behind by five years on average. 
% In addition, 
% firmware contains more and more vulnerabilities caused by TPCs over time, and 
% vendors hardly update vulnerable TPCs simultaneously when the firmware is updated. 
Besides, we explore the geographical distribution of vulnerable devices, and confirm the security situation of devices in several regions, e.g., South Korea and China, is more severe than in other regions. Further analysis shows $2,478$ commercial firmware images have potentially violated GPL/AGPL licensing terms. To facilitate future research, we will open-source our dataset.

% The analysis is based on our system 

% In summary, our work
% ,
% which plans to provide a comprehensive overview of the security situations of firmware and offer an automatic firmware analysis system, 
% can serve as an essential guideline for investigating the security of IoT firmware, and advancing the development of a more secure environment for IoT systems. We will open-source our dataset to facilitate future research.

% The recent years we have witnessed the rapid booming of IoT devices which have entered into every corners of our daily lives. Nevertheless, the core part of IoT devices, known as firmware images, may have severe security issues. 
% % IoT devices are usually equipped with the firmware images, which serve as the core of whole devices. The security of firmware images is becoming 
% % Nevertheless, the rapid development of IoT devices also significantly increases the corresponding security issues. 
% Previous works have proposed several approaches to address the critical security risks of firmware images. \yuan{\color{red}Why?}  Unfortunately, these approaches cannot apply to analyze the firmware images at large-scale since they are not scalable on different kinds of firmware images or extremely time-consuming. In addition, they mainly focus on the security of Linux based firmware images and lack the discussion on the security of firmware images wie.g., the firmware images of smart homes.
% Therefore, it is still challenging to design an effective and robust method to quickly find the vulnerabilities in firmware images at large-scale. 
% % Recent works have revealed the massive vulnerabilities in IoT devices, 
    
% \yuan{\color{red}Is there a unique angle that we can claim it to be a first study?}
% In this paper, we present \system, a first practical and scalable system that dedicates to discovering the third-party components used in firmware images and identifying the corresponding vulnerabilities.  
% Based on \system, we conduct the so far largest-scale analysis of the firmware images, which is also the first to discuss the security of tiny firmware images whose sizes are less than 1MB at large-scale. Specifically, we perform the analysis on $34,430$ firmware images across $13$ vendors including $11,000$ public accessible firmware images and $23,430$ private firmware images. 
% We successfully detect $584$ third-party components and identify a total of $128, 757$ security vulnerabilities caused by $429$ CVEs in over $34,430$ firmware images, with less than $24$ hours. We also compare the \system with two similar systems developed by 360~\cite{360iot} and Alibaba~\cite{aliiot} in $20$ test cases. \system detects an average of $11.7$ third-party components and $104.2$ vulnerabilities per firmware image while the corresponding numbers of 360 and Alibaba are $4.8$ and $62.3$, $3 and 55.5$. In addition, \system spends an average of $4.2s$ processing each firmware image while 360 spends $60s$ and Alibaba spends $174.7s$.
% % \system can identify more third-party components and detect more corresponding vulnerabilities than them with less time.
% Moreover, we reveal that the third-party components used in our collected firmware images have fallen behind by average five years.
% Finally, we explore the geographical difference in the safety standard of IoT devices. We confirm the security situation of IoT devices in several regions, e.g., Korea and China, is more severe than in other regions.
\end{abstract}




==> 0x03Setup.tex <==
\section{Dataset}
\label{Section: Dataset}

% In this section, we first give a detailed overview of our dataset. We then illustrate the comprehensive analysis results including N-days vulnerabilities we discovered.

% \subsection{Dataset Overview}
We implement a custom script to crawl firmware images from four sources: 1) official website, 2) FTP site, 3) community, and 4) private firmware repository. 
As shown in Table~\ref{Table: Dataset Composition}, we initially collect a total of $37,266$ firmware images varying from $13$ vendors, which includes $20$ kinds of devices.  More specifically, $13,328$ firmware images are crawled from the Internet, and $23,938$ firmware images are obtained from TSmart. Since our raw dataset may contain a portion of non-firmware files and the categories of a great number of firmware images are still unrecognized, we conduct a thorough data filtration on our dataset.
% After dataset filtering, we get rid of $2,836$ invalid firmwares or non-firmware files and obtain  $34, 430$ firmwares which contain XXX public accessible firmwares and XXX private firmwares from Tuya.

\textbf{Firmware Filtration} \ \ \ Identify the real firmware and filter the non-firmware files from our raw dataset are necessary to preprocess works for our following study, which require a significant amount of manual effort.

Though our script crawls the metadata in the meantime when we collect the firmware images from the Internet, we still lack enough information to identify the exact categories of a part of these public accessible firmware images. 
We first use our firmware unpacking framework to filter the non-firmware files, e.g., PE format files, that base on our maintained non-firmware file list. Next, for the remained unrecognized firmware images, we still use the framework to identify their architectures, filesystems, and operating systems, which can serve as criteria to help us identify whether they are valid firmware images. 

Then, we manually identify the device category of valid unrecognized firmware images by checking them on official websites and searching them through the Internet.
Nevertheless, there are still a great number of valid firmware images which device categories cannot be identified. We classify these valid unrecognized firmware images as \textit{unknown}.

For the firmware images collected from TSmart, we obtain a CSV file that has a brief description of each firmware. Nevertheless, the CSV file still lacks some important information, e.g., the specific category of devices, for $7,912$ firmware images.
% Based on the CSV file, it is straightforward to classify the firmwares from Tuya. 
% However, we still cannot simply identify a significant number of firmwares.
% there are still a great number of firmwares that cannot be simply identified.
% The CSV file does not provide enough information, 
Fortunately, we notice that the name of some firmware contains its purpose, e.g., Bluetooth light strip, which can be used to infer its exact category.
Thus, we manually check the name of $7,912$ firmware images and identify the categories of $2,029$ firmware images. We classify the remained $5,883$ firmware images as \textit{unknown}.

% As shown in Table~\ref{Table: Dataset}, we totally collect $34,303$ firmwares varying from 14 vendors which involve 20 kinds of devices.  $11,100$ firmwares are crawled from the Internet and $23,203$ firmwares are obtained from Tuya. 

%  \textbf{Firmware Identification and Classify.} 
% Though we obtain a great number of firmwares through the trusted sources, our firmware dataset may contain a part of  non-firmware files.
% % there is still a part of firmwares that may invalid or belong to non-firmware files. 
% Therefore, we adopt the \textit{binwalk} again to extract the objects from firmwares to determine whether they are valid firmwares. For the files which belong to the non-firmware files, the \textit{binwalk} will output the exact file types or not output any information.

\textbf{Dataset Composition} \ \ \ We list the detailed composition of our dataset as shown in Table~\ref{Table: Dataset Composition}. After dataset filtration, we get rid of $2,770$ non-firmware files and finally obtain $33,833$ firmware images across $13$ vendors including $13,173$ public accessible firmware images and $23,430$ private firmware images from TSmart. Our dataset includes a total of $19$ kinds of known IoT devices and a part of unknown IoT devices. As shown in , $6.7\%$ firmware images are used in the camera, $19.5\%$ firmware images belong to the router, $1.7\%$ firmware images are deployed on the switch, $51.2\%$ firmware images collected from TSmart have been equipped on smart homes. However, there are still $20.8\%$ firmware images for which exact device categories cannot be identified. We classify these unidentified firmware images as unknown. Apart from vendors and devices mentioned above, our dataset also covers several instruction sets, of which ARM ($84.1\%$) takes the majority, and MIPS follows ($11.1\%$). And some different filesystems are also included in the dataset, like Squashf, CramFS, etc. Despite that the embedded systems environment is heterogeneous, spanning a variety of devices, vendors, architectures, instruction sets, operating systems, and custom components, we spare no effort to build a more representative dataset.

Overall, our firmware dataset is highly representative, which contains IoT devices ranging from consumer to professional devices, such as routers, cameras, switches, smart homes, open-source firmware, and so on. Besides, the dataset includes a great number of private firmware images, which are used for research purposes for the first time. Our dataset has a larger scale and higher research value than previous studies. To facilitate future firmware security research, we will open-source a part of our dataset.
\yuan{\color{red}In this case, we will be asked about dataset release. We need to mention the dataset that we plan to release.}
    
%  \subsection{Results}
%  Our system dedicates to discovering the vulnerabilities of firmwares that caused by third-party components.
 
%  \subsubsection{Third-party Components}
 
 


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\caption{Dataset Composition}
\label{Table: Dataset Composition}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccccccc}
\hline
Vendor &
  Category &
  \begin{tabular}[c]{@{}c@{}}\# Download\\ Firmware\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\# Valid\\ Firmware\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Squashfs \\ Filesystem\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}CramFS   \\ Filesystem\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Linux EXT \\ Filesystem\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}JFFS2 \\ Filesystem\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Other\\ Filesystem\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Unknown \\ Filesystem\end{tabular} &
  ARM &
  MIPS &
  X86 &
  \begin{tabular}[c]{@{}c@{}}Unknown \\ ARCH\end{tabular} &
  Little Endian &
  Big Endian &
  Unknown Endian \\ \hline
Xiongmai                  & Camera          & 1,038 & 520  &      & 45  &    &    & 1  & 474  & 326  &     &     & 194  & 45   &     & 475   \\ \hline
Tomato-shibby             & Router          & 642  & 230  & 230  &     &    &    &    &      & 168  &     &     & 62   & 230  &     & 0     \\ \hline
Phicomm                   & Router          & 107  & 107  & 73   &     &    &    &    & 34   & 30   & 25  &     & 52   & 72   & 1   & 34    \\ \hline
Fastcom                   & Camera          & 164  & 113  &      &     &    &    &    & 113  & 53   &     &     & 60   &      &     & 113   \\ \hline
\multirow{4}{*}{Trendnet} & Camera          & 328  & 313  & 8    & 24  &    &    &    & 281  & 179  & 41  &     & 93   & 32   &     & 281   \\ \cline{2-17} 
                          & Router          & 463  & 336  & 261  &     &    &    &    & 75   & 119  & 91  &     & 126  & 221  & 40  & 75    \\ \cline{2-17} 
                          & Switch          & 162  & 162  & 93   &     &    & 18 &    & 51   & 116  & 17  &     & 29   & 80   & 31  & 51    \\ \cline{2-17} 
                          & Unknown         & 414  & 352  & 16   & 39  &    & 5  &    & 292  & 252  & 71  &     & 29   & 54   & 6   & 292   \\ \hline
Xiaomi                    & Router          & 21   & 21   & 21   &     &    &    &    &      & 8    & 9   &     & 4    & 21   &     &       \\ \hline
\multirow{4}{*}{TP-Link}  & Camera          & 256  & 354  &      &     & 10 & 3  &    & 165  & 128  &     & 1   & 370  &      & 12  &       \\ \cline{2-17} 
                          & Router          & 482  & 272  &      &     & 17 &    & 10 & 61   & 346  & 3   & 34  & 272  & 1    & 194 & 12    \\ \cline{2-17} 
                          & Switch          & 185  & 205  &      &     &    &    &    & 89   & 10   &     & 150 & 227  &      & 80  & 121   \\ \cline{2-17} 
                          & Unknown         & 514  & 136  &      &     & 28 & 3  & 16 & 52   & 332  &     & 66  & 137  & 7    & 127 & 19    \\ \hline
\multirow{4}{*}{D-Link}   & Camera          & 326  & 326  & 15   & 8   &    &    &    & 303  & 167  & 106 &     & 53   & 23   &     & 303   \\ \cline{2-17} 
                          & Router          & 356  & 353  & 269  &     &    & 2  &    & 82   & 180  & 83  & 4   & 86   & 214  & 57  & 82    \\ \cline{2-17} 
                          & Switch          & 542  & 212  & 146  &     &    &    &    & 66   & 177  & 5   & 1   & 29   & 129  & 17  & 66    \\ \cline{2-17} 
                          & Unknown         & 976  & 655  & 231  & 22  &    & 4  &    & 398  & 236  & 34  & 3   & 382  & 174  & 83  & 398   \\ \hline
Hikvision                 & Camera          & 158  & 139  &      & 47  &    & 1  &    & 91   & 131  &     &     & 8    & 48   &     & 91    \\ \hline
Foscam                    & Camera          & 113  & 113  &      &     &    &    &    & 113  & 53   &     &     & 60   &      &     & 113   \\ \hline
Dahua                     & Camera          & 419  & 419  & 9    & 19  & 2  &    & 1  & 388  & 260  & 2   & 1   & 156  & 28   &     & 391   \\ \hline
\multirow{17}{*}TSmart    & Sweeper         & 33   & 33   &      &     &    &    & 1  & 32   & 12   &     &     & 21   &      &     & 33    \\ \cline{2-17} 
                          & Lightstrip      & 6,403 & 6,373 &      &     &    &    &    & 6,373 & 364  &     &     & 6,009 &      &     & 6,373  \\ \cline{2-17} 
                          & General         & 1,107 & 1,092 & 13   &     &    & 41 &    & 1,038 & 225  & 13  &     & 854  & 54   &     & 1040  \\ \cline{2-17} 
                          & Plugin          & 7,775 & 7,697 &      &     &    &    &    & 7,697 & 367  &     &     & 7,330 &      &     & 7,697  \\ \cline{2-17} 
                          & Heater          & 340  & 339  &      &     &    &    &    & 339  &      &     &     & 339  &      &     & 339   \\ \cline{2-17} 
                          & Blueteeth Light & 1,457 & 977  &      &     &    &    &    & 977  & 637  &     &     & 340  &      &     & 977   \\ \cline{2-17} 
                          & Air             &      & 456  &      &     &    &    &    & 456  & 96   &     &     & 360  &      &     & 456   \\ \cline{2-17} 
                          & Curtain         & 115  & 115  &      &     &    &    &    & 115  & 8    &     &     & 107  &      &     & 115   \\ \cline{2-17} 
                          & Lock            & 51   & 51   &      &     &    &    &    & 51   &      &     &     & 51   &      &     & 51    \\ \cline{2-17} 
                          & Freezer         & 40   & 40   &      &     &    &    &    & 40   &      &     &     & 40   &      &     & 40    \\ \cline{2-17} 
                          & Air Purifier    & 24   & 24   &      &     &    &    &    & 24   &      &     &     & 24   &      &     & 24    \\ \cline{2-17} 
                          & Humidifier      & 12   & 12   &      &     &    &    &    & 12   &      &     &     & 12   &      &     & 12    \\ \cline{2-17} 
                          & Dehumidifier    & 55   & 55   &      &     &    &    &    & 55   &      &     &     & 55   &      &     & 55    \\ \cline{2-17} 
                          & Heat Controller & 34   & 33   &      &     &    &    &    & 33   &      &     &     & 33   &      &     & 33    \\ \cline{2-17} 
                          & Fan             & 19   & 19   &      &     &    &    &    & 19   &      &     &     & 19   &      &     & 19    \\ \cline{2-17} 
                          & Washer          & 4    & 4    &      &     &    &    &    & 4    & 4    &     &     &      &      &     & 4     \\ \cline{2-17} 
                          & Unknown         & 5,883 & 5,883 & 167  & 147 &    & 74 &    & 5,494 & 1,349 & 52  & 1   & 4,481 & 378  &     & 5,505  \\ \hline
OpenWrt                   & Unknown         & 5,585 & 5,292 & 3,903 &     & 12 & 41 & 55 & 1,281 & 2,415 & 194 & 10  & 2,673 & 3,865 & 79 & 1,348 \\ \hline
\end{tabular}%
}
\end{table*}

==> 0x05CaseStudies.tex <==
\section{Case study}
% In this section, we conduct a case study on the impact of two well-known vulnerabilities: \textit{OpenSSL} Heartbleed vulnerability  (CVE-2014-0160) and \textit{glibc}  GHOST  vulnerability  (CVE-2015-0235) on our dataset.


% As shown in Table~\ref{Table: Firmware images affected by two vulnerabilities}, we find these two vulnerabilities have affected 604 firmware images which account for $1.8\%$ of the dataset. More specifically, 380 firmware images from 8 vendors are vulnerable to the Heartbleed vulnerability and 224 firmware images from 4 vendors contain the GHOST vulnerability. TP-Link has the most vulnerable firmware images that affected by two vulnerabilities. Besides, we have explored the release dates of these vulnerable firmware images. We discover that all firmware images that affected by the Heartbleed vulnerability were released after the vulnerability was disclosed, and only 7 firmware images that affected by the GHOST vulnerability were released before the vulnerability was disclosed.




% \section{Case Studies}
% To further provide  new insights of IoT firmwares, we present a case study in this section.

% % \subsection{Performance Measurement}
% % In this subsection, we explore the 

% % \subsection{Performance Measurement}
% % \label{section: performance measurement}
% % The \system achieves great results in matching the third-party components and identifying the N-days vulnerabilities from $34,430$ firmwares. Currently, we find several companies also provide similar tools that can detect the N-days vulnerabilities from the firmwares and most of these tools are still in test.
% % In this subsection, to measure the performance of \system, we compare our system with the tools from 360~\cite{360iot} and Alibaba~\cite{aliiot} which are still beta versions. 

% % The 360 offers unlimited free trials to the public, however, Alibaba only offers one free trial for us.  Though Alibaba's tool is still in test, it charges \$300 for each extra test. Due to the limit budget, we purchase extra $21$ usage times which costs us $\$6,300$. As shown in Table~\ref{Table: Comparison}
% % , we select representative $21$ firmwares from six vendors as test cases.  The \system goes beyond the other two systems in several aspects. 

% % First of all, except for the smart light from Tuya, \system can successfully analyze all firmwares while 360 cannot deal with $2$ firmwares and Alibaba lacks the results of $6$ firmwares.  Those firmwares that cannot be analyzed by 360 and Alibaba do not adopt the traditional file systems which increase the difficulty of analysis.
% % In addition, to measure the performance of \system comprehensively, we specially select a firmware from Tuya which cannot be analyzed by \system. 
% % Expectedly, 360 and Alibaba also cannot handle this firmware.

% % \textbf{TODO} Second, \system detects the most third-party components in all firmwares among the three systems.  
% % % The \system maintains a large scale vulnerability list to match the third-party components in firmwares.  
% % The \system has discovered all the third-party components with the same version that reported by 360 and Alibaba. Since \system maintains a large scale vulnerability list and adopt用s the natural language process and regular expression based matching method, 
% %  it discovers more third-party components which contain confirmed N-days vulnerabilities than 360 and Alibaba. 

% % Third, \system identifies more N-days vulnerabilities in xx of xx test cases in comparison with other two systems. The \system mainly depends on CVE Detail~\cite{cvedetail} to collect the N-days vulnerabilities. Though we identify all the third-party components with the same version that discovered by 360 and Alibaba, we still find fewer vulnerabilities than them. 
% % Based on our investigation, we realize that 360 and Alibaba maintain their own vulnerability datasets, which contain more detailed vulnerability information of third-party components than CVE Detail. For example, for the firmware of  3001\_tew755ap\_fw102b06.bin
% % from Trendnet, \system and Alibaba both detect the \textit{tcpdump} used in the firmware. Nevertheless, the CVE Detail only provides us the corresponding N-days vulnerabilities from 2018 to 2019 while Alibaba reports the vulnerability since 2014.
% % Besides, their results contain a part of incorrect N-days vulnerabilities which not belong to the corresponding firmwares.
% % Therefore, we conduct further study to ensure our experiments are implemented fairly. We use the same vulnerability dataset based on CVE Detail for three systems. The vulnerabilities that found by 360 and Alibaba decreased dramatically after we change the vulnerability dataset . With the same vulnerability dataset, \system discovers more N-days vulnerabilities than 360 and Alibaba in all test cases since we can detect more third-party components.

% % Overall, our results show that \system has a much better performance than the systems from two well-known companies 360 and Alibaba. With our custom third-party components list and the same vulnerability dataset, we can detect more third-party components and dig out more N-days vulnerabilities than them.

% % \subsection{Geographical Difference}

% % Previous work~\cite{kumar2019all} indicates that IoT device security varies greatly with geographical changes. Thus, we conduct two experiments to explore whether vendors adopt different security strategies in different regions.

% % First of all, we split the firmwares from TP-Link into two versions: TP-Link\_EN and TP-Link\_ZH, based on the way we collected. The firmwares from TP-Link\_EN are mainly released on the United States and Europe, and the firmwares from TP-Link\_EN are deployed on China. 
% % As shown in Table~\ref{Table: TP-Link}, for each category of devices, the firmwares from TP-Link\_ZH contain more vulnerabilities than that from TP-Link\_EN.
% % % Though we divide them into two parts, they still serve the same functions if they belong to the same category. 
% % For example, the cameras from TP-Link\_EN have an average of $86.06$ vulnerabilities while that from TP-Link\_zh contain an average of $4.5$ vulnerabilities. 
% % What's more, \system can detect more third-party components from TP-Link\_ZH than TP-Link\_EN which indicates that the firmwares from TP-Link\_CN are more vulnerable.
% % % Further, we notice that these two versions of products adopt the different third-party components in developing the same kinds of IoT devices. 
% % % For instance, we only detect 


% % Second, we figure out the number of vulnerable IoT device in each country or region. We select 455 different models of IoT devices, e.g., DIR-827 from D-Link and TL-IPC423 from TP-Link, which corresponding firmwares are included in our dataset and have been confirmed to have vulnerabilities. Then, we utilize the \textit{Shodan}~\cite{shodan} to find the distribution of these possible vulnerable IoT devices. \textit{Shodan} is a well-known IoT search engine that can search the IoT devices exposed to the Internet.
% % We create a heat map which is based on the number of vulnerable IoT devices in each country or region, as shown in Figure~\ref{Figure: Risk Heat Map}. 
% % Asia contains six of the top 10 riskiest regions in the world, which are Korea, Taiwan, Singapore, China and Hongkong and the United Arab Emirates. What's more, Korean contains the most vulnerable IoT devices in the world, which reaches $20,191$.
% % Europe contains relatively few vulnerable IoT devices, though Sweden and Italy are two of the top 10 riskiest regions in the world.
% % The United States and Canada, which belong to the North America, have a large number of vulnerable IoT devices.  The United States contains $9,430$ vulnerable IoT devices, which just fewer than Korea.
% % % In Asia,  are the top 5 highest risk areas. What's more, Korea contains the most vulnerable IoT devices in the world.
% % % . In 
% % % What's more, the North America, including the United States and Canada, 

% % % We finally get two types of data, one is the number of vulnerable IoT devices in each country or region, the other one is the total number of IoT devices from corresponding vendors in the same country or region.
% % % We calculate the risk score by dividing these two types of data and present the results in a heat map, as shown in Figure~\ref{Figure: Risk Score Heat Map}.

% % % We also obtain the total number of IoT devices of corresponding vendors, which are exposed to the Internet, in each country or region. We get the risk score by simply . 

% % % We create a risk score heat map for each country and region, as shown in Figure~. Korean has the highest risk score which reaches $6730$.  
% % % The countries and regions in Europe have lower risk scores than in Asia.
% % % In addition, more firmwares from TP-Link\_zh  can be analyzed by \system, which means that they are more vulnerable to attack.
% % % In addition, according to \textit{Tuya}, the European Union has a much higher security and privacy






% % % %%Begin: Figure: the Architecture of XXX
% % % \begin{figure}
% % % % \centering
% % % \includegraphics[width=0.50\textwidth]{Figures/CVEMap.eps}
% % % \caption{World Map of Vulnerable IoT Devices}
% % % \label{Figure: Risk Heat Map}
% % % \end{figure}
% % % %%End: Figure: Vulnerable Rate Trending of Route


% % \begin{figure*}
% %   \centering
% %   \subfigure[World Map of Vulnerable IoT Devices]
% %   {
% %   \begin{minipage}[b]{0.4\textwidth}
% %     \label{Figure: Risk Heat Map} %% label for first subfigure
% %     \includegraphics[width=\textwidth]{Figures/CVEMap.eps}
% %   \end{minipage}
% %   }
% %   \hspace{1in}
% %   \subfigure[Top 10 Regions with the Most Vulnerable IoT Devices]{
% %   \begin{minipage}[b]{0.4\textwidth}
% %     \label{Figure: Top 10 Regions} %% label for second subfigure
% %     \includegraphics[width=\textwidth]{Figures/VulneraableIoTDeviceRegion.eps}
% %     \end{minipage}
% %     } 
% %   \caption{World Distribution of Vulnerable IoT Devices}
% %   \label{Figure: World Map} %% label for entire figure
% % \end{figure*}




==> 0x09CaseStudy.tex <==
\section{Case study}
In this section, we conduct a case study on the impact of two well-known vulnerabilities: OpenSSL Heartbleed vulnerability  (CVE-2014-0160) and glibc  Ghost  vulnerability  (CVE-2015-0235) on our dataset.

==> 0x0Challenges.tex <==
% \section{Overview}


==> 0x0RelatedWork.tex <==
% \section{related work}
% Costin et al.~\cite{costin2014large} conducted the first large-scale analysis of firmwares based on their frameworks. They proposed a correlation technique to find similar firmwares by propagating vulnerability information.


% \textbf{Firmware Unpacking.} Unpacking firmwares is a known problem, and
% several tools for this purpose exist. Binwalk~\cite{binwalk} is a firmware analysis toolbox that provides various methods
% and tools for extraction, inspection and reverse engineering
% of firmwares or other binary blobs. FRAK
% is a framework to unpack, analyze, and repack firmware
% images of embedded devices. FRAK was never publicly
% released and reportedly supports only a few firmware formats
% (e.g., Cisco IP phones and IOS, HP laser printers).
% The Binary Analysis Toolkit (BAT) was originally
% designed to detect GPL license violations, mainly
% by comparing strings in a firmware to strings
% present in open source software distributions. For this
% purpose BAT has to unpack firmwares. Unfortunately,
% as we show in Section 3, none of these tools are
% accurate and complete enough to be used as is in our
% framework.

% \textbf{Firmware Analysis} There are many examples of security analysis of embedded
% systems. Several network card firmwares
% have been analyzed and modified to insert a backdoor
% or to extend their functionality . Davidson
% et al.  propose FIE, built on top of the KLEE symbolic
% execution engine, to incorporate new symbolic execution
% techniques. It can be used to verify security properties
% of some simple firmwares often found in
% practice. Zaddach et al.  describe Avatar, a dynamic
% analysis platformfor firmware security testing. In Avatar,
% the instructions are executed in an emulator, while the IO
% accesses to the embedded system’s peripherals are forwarded
% to the real device. This allows a security engineer
% to apply a wide range of advanced dynamic analysis
% techniques like tracing, tainting and symbolic execution.

% A large set of firmwares of Xerox devices were
% reverse-engineered by Costin leading to the discovery
% of hidden PostScript commands. Such commands allow
% an attacker to e.g., dump a device’s memory, recover
% passwords, passively scan the network and more generically
% interact with devices’ OS layers. Such attacks could
% be delivered to printers via web pages, applets, MSWord
% and other standard printed documents .

% Bojinov et al. conducted an assessment of the security
% of current embedded management interfaces. The
% study, conducted on real physical devices, found vulnerabilities
% in 21 devices from 16 different brands, including
% network switches, cameras, photo frames, and lightsout
% management modules. Along with these, a new class
% of vulnerabilities was discovered, namely cross-channel
% scripting (XCS) . While XCS vulnerabilities are not
% particular to embedded devices, embedded devices are
% probably the most affected population. In a similar study,
% the authors manually analyzed ten Small Office/Home
% Office (SOHO) routers  and discovered at least two
% vulnerabilities per device.

% Looking at insecure (remote) firmware updates, researchers
% reported the possibility to arbitrarily inject
% malware into the firmware of a printer.
% Chen  and Miller  presented techniques and implications
% of exploiting Apple firmware updates. In a
% similar direction, Basnight et al.  examined the vulnerability
% of PLCs to intentional firmware modifications.
% A general firmware analysis methodology is presented,
% and an experiment demonstrates how legitimate firmware
% can be updated on an Allen-Bradley ControlLogix L61
% PLC. Zaddach et al.  explore the consequences of a
% backdoor injection into the firmware of a hard disk drive
% and uses it to exfiltrate data.
% French and Casey present fuzzy hashing techniques
% in applied malware analysis. Authors used
% ssdeep on CERT Artifact Catalog database containing
% 10.7M files. The study underlines the two fundamental
% challenges to operational usage of fuzzy hashing at scale:
% timeliness of results, and usefulness of results. To reduce
% the quadratic complexity of the comparisons, they propose
% assigning files into “bins” based on the block and
% file sizes. This approach, for their particular dataset and
% bins partitioning strategy, allowed for a given fuzzy hash
% to reduce the search space on average by 83.1\%.
% Finally, Bailey et al.  and Bayer et al. propose
% efficient clustering approaches to identify and groupmalware
% samples at large scale. Authors perform dynamic
% analysis to obtain the execution traces of malware programs
% or obtain a description of malware behavior in
% terms of system state changes. These are then generalized
% into behavioral profiles which serve as input to an
% efficient clustering algorithm that allows authors to handle
% sample sets that are an order of magnitude larger than
% previous approaches. Unfortunately, this approach cannot
% be applied in our framework since dynamic analysis
% is unfeasible due to the heterogeneity of architectures
% used in firmwares.

==> backup.tex <==
\begin{table*}[]
\caption{Analysing Results of Our Dataset}
\label{Table: Vulnerability}
\centering
\begin{tabular}{cccccccc}
\hline \hline
Vendor &
  Category &
    \begin{tabular}[c]{@{}c@{}}\# Valid \\ Firmware\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}\# Identified \\ Firmware\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\# Third-party \\ Components\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\# Average \\ Third-party Components\end{tabular} &
  \# Vulnerabilities &
  \begin{tabular}[c]{@{}c@{}} \# Average \\ Vulnerabilities\end{tabular} \\ \hline
Xiongmai                  & Camera      & 520    & 195   & 232     & 1.19  & 313    & 1.61  \\ \hline
Tomato-shibby             & Router      & 230    & 230   & 2,088   & 9.08  & 11,948 & 51.95 \\ \hline
Phicomm                   & Router      & 107    & 97    & 405     & 4.18  & 1,818  & 18.74 \\ \hline
Fastcom                   & Router      & 113    & 85    & 199     & 2.34  & 1,093  & 9.67  \\ \hline
\multirow{4}{*}{Trendnet} & Camera      & 313    & 32    & 58      & 1.81  & 665    & 20.78 \\ \cline{2-8} 
                          & Router      & 336    & 305   & 1,762   & 5.78  & 7,903  & 25.91 \\ \cline{2-8} 
                          & Switch      & 162    & 117   & 366     & 3.13  & 3,157  & 26.98 \\ \cline{2-8} 
                          & Unknown     & 352    & 57    & 137     & 2.40  & 1,962  & 34.42 \\ \hline
Xiaomi                    & Router      & 21     & 20    & 251     & 12.55 & 2,440  & 122   \\ \hline
\multirow{4}{*}{TP-Link}  & Camera      & 256    & 236   & 1,625   & 6.89  & 19.494 & 82.60 \\ \cline{2-8} 
                          & Router      & 482    & 441   & 3,935   & 8.92  & 25,821 & 58.55 \\ \cline{2-8} 
                          & Switch      & 185    & 3     & 20      & 6.67  & 134    & 44.67 \\ \cline{2-8} 
                          & Unknown     & 514    & 279   & 1,127   & 4.04  & 14,159 & 50.75 \\ \hline
\multirow{4}{*}{Dlink}    & Camera      & 326    & 16    & 85      & 5.31  & 711    & 44.44 \\ \cline{2-8} 
                          & Router      & 353    & 285   & 2,296   & 8.06  & 11,810 & 41.44 \\ \cline{2-8} 
                          & Switch      & 212    & 0     & 0       & 0     & 0      & 0     \\ \cline{2-8} 
                          & Unknown     & 655    & 222   & 940     & 4.23  & 6,933  & 31.23 \\ \hline
Hikvision                 & Camera      & 139    & 2     & 8       & 4     & 127    & 63.5  \\ \hline
Foscam                    & Camera      & 113    & 0     & 0       & 0     & 0      & 0     \\ \hline
Dahua                     & Camera      & 419    & 11    & 43      & 3.91  & 430    & 39.09 \\ \hline
TSmart                      & Smart Homes & 23,330 & 438   & 856     & 1.95  & 4,353  & 9.94  \\ \hline
OpenWrt                   & Unknown     & 5,292   & 4,940 & 300,020 & 60.73 & 13,486 & 2.73  \\ \hline \hline
\end{tabular}
\end{table*}


